Sublinear Elliptic Operators

We investigate second order elliptic equations \[F(\mathcal{H}u) = 0\] where the function $F\colon S(n)\to\mathbb{R}$ on the space of symmetric $n\times n$ matrices is assumed to be sublinear. There is very little to be found in the literature devoted particularly to sublinear elliptic operators. When examples of such operators occur, they are often merely treated as members of the larger class of convex operators. That class has been thoroughly investigated and many of its aspects are well understood. There is, however, something to be said about sublinear operators that do not, in general, apply to convex operators.

==> sublin/jensens_lem.tex <==
Recall the definition of semiconcave functions, the convex envelope, and the contact set on page \pageref{semicondef}.
\begin{lemma}[Jensen]\label{jensen}
Let \(D\subseteq\mathbb{R}^n\) be open and bounded and let \(w\colon\overline{D}\to\mathbb{R}\) be semiconcave.
If the minimum of \(w\) is \emph{not} on the boundary, i.e.
\[\min_{\overline{D}} w < \min_{\partial D} w,\]
then the contact set \(\mathcal{A}(w)\) has positive measure.
\end{lemma}

\begin{proof}
We may assume that the minimum value is obtained at the origin and is 0. That is
\[0 = w(0),\qquad 0\in D,\qquad w|_{\partial D} \geq \delta > 0.\]
Write
\[d := \operatorname{diam}(D) = \sup\{|x-y|\;:\;x,y\in D\} < \infty.\]
Let \(q\in\mathbb{R}^n\) with length \(|q|<\frac{\delta}{d}\). Then
\[a := \min_{x\in\overline{D}} \big(w(x) - q^Tx\big) = w(x_0) - q^Tx_0 \leq 0,\qquad x_0\in D,\]
since \(w(0) = 0\) and for \(\eta\in\partial D\) we have
\[w(\eta) - q^T\eta \geq \delta - |q||\eta| > \delta - \frac{\delta}{d}d = 0.\]
Thus \(\phi(x) := a + q^Tx\) touches \(w\) from below at the interior point \(x_0\).
This means that \(x_0\in \mathcal{A}\).

Since \(\Gamma(x) \leq w(x)\) with equality at \(x_0\) and since \(w\) is semiconcave, \(\Gamma\) is touched both above and below at \(x_0\) by smooth functions. This implies that \(\Gamma\) is differentiable at \(x_0\) and that
\[\nabla\Gamma(x_0) = \nabla\phi = q^T.\]
Defining the image set
\[\nabla\Gamma(\mathcal{A}) := \{\nabla\Gamma(x)\;|\; x\in\mathcal{A}\},\]
we have proved that
\begin{equation}
B\left(0,\delta/d\right) \subseteq \nabla\Gamma(\mathcal{A}).
\label{ballnabla}
\end{equation}

Since \(\Gamma\) is convex, the gradient \(\nabla\Gamma\) is differentiable a.e. in \(\Omega\). In \(\mathcal{A}\), \(\Gamma\) is touched above by a paraboloid with Hessian \(\mu I\). Thus the Alexandrov derivative of the gradient satisfies
\begin{equation}
D[\nabla\Gamma^T] = \mathcal{H}\Gamma \leq \mu I\qquad\text{a.e. in }\mathcal{A}.
\label{abnd}
\end{equation}
By change of variables, \(y = \nabla\Gamma(x)\), equation \eqref{ballnabla} and \eqref{abnd} implies (må også muligens vise at \(\nabla\Gamma\) er Lipschitz)
\begin{align*}
0 &< |B(0,\delta/d)|\\
                        &\leq |\nabla\Gamma(\mathcal{A})|\\
												&= \int_{\nabla\Gamma(\mathcal{A})}\dd y\\
												&= \int_{\mathcal{A}}|\det D[\nabla\Gamma^T(x)]|\dd x\\
												&= \int_{\mathcal{A}}|\det \mathcal{H}\Gamma|\dd x\\
												&\leq \mu^n|\mathcal{A}|.
\end{align*}
Thus \(|\mathcal{A}|>0\).
\end{proof}


